A Blueprint for Public Engagement Appraisal: Supporting Research Careers

Time spent performing public engagement is severely undervalued by research institutions around the globe. In this article we present one possible system that could be implemented to provide researchers with career recognition for performing this vital work. The framework utilises the supervision system that is already in place at many research institutions, whereby senior researchers mentor their junior colleagues. This would encourage more researchers to engage with the public, as well as increasing the quality of this engagement.

==> conclusion.tex <==
\section{Conclusion}

There clearly is an issue within research institutions at the moment. Projects not relevant to published research are undervalued, especially with public engagement. We believe that our goal-setting and assessment framework can go some way to fixing this problem, but this really depends on the institution.

Institutions that want to increase their public engagement output must be committed to fostering a pro-engagement atmosphere, along with the researchers within them. For this, there may need to be some extra training provided to researchers and individuals must not feel pressured into performing public engagement initiatives. Whilst this is the ``third aim", requiring public engagement could lead to extreme dissatisfaction and terrible experiences from the public's point of view. However, any individual who wants to engage should be welcomed with open arms and supported by the institution.


==> framework.tex <==
\section{Goal setting and public engagement}
\label{sec:frame}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=\textwidth]{media/flowchart_goalsetting_v3.pdf}
    \caption{General outline of the goal-lead public engagement framework. The secondary meeting may need to take place more than once, depending on the scale of the project.}
    \label{fig:goal_setting_pe}
\end{figure*}

It is clear that research institutions would like more outreach to be performed, not just because of the personal interests of staff within the institution, but because of the wealth of benefits such activities bring \citep{why_lock}. Currently, the only way that performance is measured within these institutions is the amount of articles published.

To increase engagement, and to ensure that practitioners receive the recognition that they deserve for work that is historically undervalued, there needs to be a proper evaluation framework in place. We suggest that this framework is worked into the current performance review system already present at most research institutions. This system, as well as increasing recognition for public engagement, should also increase the quality of such exercises by acting as a motivational tool and support network.

It must be noted that for such a system to be truly effective, the research institution must be fully committed. There is no point in collecting all of this data and then forgetting about public engagement when discussing career opportunities. This is a fantastic way for institutions to realise their ``third aim" and should be treated similarly to other evaluation and support programmes. However, there is some research to suggest that salary benefits and support for future initiatives should not be contained in the same meeting, as this will lead to an extreme time bias towards discussing salary benefits \citep{pm_pula}.

Below we outline an example of a system that would implement a career recognition system for practitioners of public engagement.

\subsection{Outline}

The two main aims of this scheme are to provide career recognition and to support scientists. It is important that the latter of these two aims is not forgotten, as it is the key to success.

To include public engagement in performance reviews, we must be able to review the activities that an individual has undertaken. These activities then must be summatively evaluated and a conclusion about the individual's performance achieved. To do this, we suggest that the following rough outline (Figure \ref{fig:goal_setting_pe}). Of course, this general framework should be modified to fit with the individual organisation for which it is being implemented.

One of the key ideas at the core of this system is continual evaluation. Without a solid evaluation framework, % more here

\subsection{Initial advisor meeting}

We suggest that this meeting is used to extend the current performance review meeting. However, if this is not possible, then of course this system can be self-contained.

Firstly, the scientist will outline their previous public engagement work and present any reports that they have created. Clearly, it is difficult to perform any kind of appraisal without such a report. However, if one does not exist, with a clear reason why (for example this is the first year the scheme has taken place), then this should not count against the academic. We are trying to encourage participation in public engagement, not participation in extra administrative work.

This report should then be evaluated by the supervisor similarly to how other projects (e.g. lecture courses) are evaluated within the institution. It is best to continue with the same general structure as previously, to avoid 'reinventing the wheel'. This would simply create confusion, and if the old system is tried and tested, there is no reason to change it.

After the summative evaluation has been completed, the initial evaluation for the next project can take place.

This will involve choosing a guiding value that aligns with that of the organisation, and setting goals that are in line with this. Here, the scientist should be given a good deal of control, as long as the goals are SMART. In this case, the R (for reasonable) is extremely important. Bad experiences where ambitious scientists overstretch themselves may lead to a short-term increase in public engagement productivity but will create an anti-engagement atmosphere.

It is also important to pitch these activities correctly, and this thought and planning should take place at this stage. For example:

\begin{itemize}
\item Who is our target audience?
\item How much time am I willing to devote to this project?
\item Is there anyone we can collaborate with?
\end{itemize}

Performing this initial evaluation will lead to higher productivity in the long term due to more focused goals.

\subsection{Planning}

In this stage, it is helpful to write out the actions that are going to help realise the outlined goals. It is important that these actions are SMART, similar to the goals, however this time the emphasis should be on the T (timed). Timed actions act as a motivator as well as a director.

Once actions are planned, work can begin. The work that should be performed at first should be preliminary, for example:
\begin{itemize}
\item Check with venues if space is available if giving a public talk
\item Write notes on the topic you are working on
\item Roughly plan the speech you are going to give
\end{itemize}

\subsection{Advisor meeting(s)}

Depending on the scale of the project, there may need to be more than one of these. Here is where the interim evaluation will take place. This is extremely important to ensure that the project stays on track and does not drift from the original goals that were laid out in the first advisor meeting.

However if there is clearly an issue with the project, then this is the stage to remedy it. These meetings are the perfect time to talk through what has gone well so far in the project, and to fix what has gone wrong. The advisor should make suggestions, including offering extra training to the scientist if required. Extra resources should also be made available if the scientist asks for them (e.g. travel expenses).

\subsection{Implementation}

After the final advisor meeting, the activity should take place. Again, depending on the project, there may be many implementations.

Once the activity has been completed, then there should be a summative evaluation. There should be reference throughout all stages of the report to the goals that were set out in the initial advisor meeting. The final report, as well as containing the initial and interim evaluation, should focus on if these goals were realised. This realisation should be documented - why were the goals realised? Why weren't they completed on time?

The report that is produced can then be shown at the next initial advisor meeting to begin the new year. Previous years should guide the next year's work.

==> introduction.tex <==
\section{Introduction}
\label{sec:intro}

Despite a large number of research institutions describing public outreach or public engagement as their third aim behind research and teaching, this engagement is usually performed by a small self-selected group of people. These researchers usually believe that it is their moral duty to perform public engagement, rather than seeing it as part of their career \citep{ind_ner}.

There is also research that suggests one of the main reasons that people do not engage with the public is that they cannot receive career recognition for doing so \citep{view_mat, car_wat}. There is no reason why they would (apart from their own personal values) go out and engage the public when they could be inside producing more papers and raising their \emph{h}-index. This is encouraged by the current `publish or perish' attitude in academia.

Not only is this attitude outdated, it is losing what public approval it has left. The role of researchers and academics in society is changing considerably. Researchers are no longer simply around to discover things about fundamental science, but they perform an important function in giving back to the world. One example is the large chunks of code (see SciPy) that are produced by researchers that can be used by other institutions, industry and the public often for free. Another is, of course, public engagement. Not only are there clear benefits for the institutions themselves \citep{why_lock}, but is there also not a moral duty to give back something to the people whose own work produces a large amount of the funding that pays for your research?

This attitude of not including participation in public engagement in career development is especially clear when looking at job descriptions. As of July 2015, out of 34 research positions on the American Astronomical Society job register (from PhD to permanent professor), only one has a single mention of outreach in it. The institution noted that they employ people to do outreach. There was no mention of this being part of the researcher's job, which is in severe conflict with the `third aim' we outlined above. It is particularly surprising to see this when in the same job descriptions there were mentions of, among other things, the quality of public transport in the town where the institution is located.

Whilst there is research that suggests the opposite, that researchers are not motivated to engage by the prospect of it contributing to the advancement of their career, these surveys tend to have very small self-selected samples and as such cannot be used to draw conclusions \citep{view_bes, fact_pol}.

Another issue is that there is still a negative attitude towards researchers who perform public engagement from their peers \citep{bio_phys}. This anti-engagement atmosphere is usually perpetuated by more senior colleagues who insist more junior researchers are `wasting their time' with public engagement. There does not seem to be any institutional resistance to this attitude on a high level, even though more people are being employed as outreach professionals. Whilst this increased employment is a step in the right direction, not tackling the underlying issue of the anti-engagement atmosphere is misguided. This atmosphere still persists despite a large number of individual researchers having a positive view towards public engagement \citep{surv_niel}.

If our aim is to engage the public, then we need to motivate researchers to do so. For this to work effectively, we also need to foster a pro-engagement atmosphere. Both of these issues can be remedied by introducing a performance review-like system in which public engagement work performed by researchers is evaluated, allowing for this to contribute to their career development.
